The semiclassical stability of de Sitter spacetime

de Sitter spacetime and Bunch-Davies vacuum are a solution to the semiclassical Einstein-Schroedinger equations describing the evolution of spacetime geometry and a massive scalar quantum field with arbitrary coupling to curvature. The stability of this solution is proven by calculating the renormalized energy momentum tensor expectation value for small spatially homogeneous deviations from the de Sitter - Bunch-Davies system and solving the linearized backreaction problem. A renormalization scheme is developed. All momentum integrations are carried out analytically. The general solution is given in terms of its Laplace transform. It contains only two artificial instabilities: a constant gauge mode and an instability on the Planck time scale lying outside of the scope of our semiclassical theory.

==> cbt.tex <==
\noindent
{\pagestyle{empty}
June 1994 \\
\vspace{3cm}
\begin{center}
 {\Large\bf The semiclassical stability\\
              of de~Sitter spacetime}\\
 \vspace{2.5cm}
 C. Busch \bigskip\\
 Institut f\"ur Theoretische Physik, Universit\"at Hannover \\
 Appelstr. 2, D-30167 Hannover, Germany \\
 \vspace{2.5cm}
 {\large\bf Abstract}\bigskip\\
 \parbox{12.5cm}{\small
  The semiclassical Einstein-Schr\"odinger equations describing the evolution
  of spacetime geometry and a massive scalar quantum field with arbitrary
  coupling to curvature are linearized around their de~Sitter -- Bunch-Davies
  solution. The renormalized energy momentum tensor expectation value is
  calculated in linear order for a spatially homogeneous deviation from the
  de~Sitter -- Bunch-Davies system. The momentum integrations are executed
  analytically. The linearized backreaction problem is completely solved via
  Laplace transformation and the general solution is analyzed with respect
  to instabilities. There are only two potential instabilities:
  a constant mode which is just a pure gauge and an instability on the Planck
  time scale which lies outside of the scope of our semiclassical theory.}
\end{center}
\vfill
\ref{nopages} pages, 3 figures
\pagebreak


Proposed running head:\\[1cm]
\hspace*{1cm}``The semiclassical stability \ldots ''\\[6cm]
Mailing address of the author:\\[1cm]
\hspace*{1cm}\parbox[t]{6cm}{      Dr. C. Busch\\
                                   B\"uckelsberg 1e\\
                                   D-46286 Dorsten\\
                                   Germany\\[5mm]
       \begin{tabular}{@{}ll} Tel.: & (49)\,2369\,6752\\
                              or    & (49)\,2362\,93\,8726\\
                              Fax:  & (49)\,2362\,93\,8766
       \end{tabular}}
}
